Text Recognition in Real Scenarios with a Few Labeled Samples

Scene text recognition (STR) is still a hot research topic in computer vision field due to its various applications. Existing works mainly focus on learning a general model with a huge number of synthetic text images to recognize unconstrained scene texts, and have achieved substantial progress. However, these methods are not quite applicable in many real-world scenarios where 1) high recognition accuracy is required, while 2) labeled samples are lacked. To tackle this challenging problem, this paper proposes a few-shot adversarial sequence domain adaptation (FASDA) approach to build sequence adaptation between the synthetic source domain (with many synthetic labeled samples) and a specific target domain (with only some or a few real labeled samples). This is done by simultaneously learning each character's feature representation with an attention mechanism and establishing the corresponding character-level latent subspace with adversarial learning. Our approach can maximize the character-level confusion between the source domain and the target domain, thus achieves the sequence-level adaptation with even a small number of labeled samples in the target domain. Extensive experiments on various datasets show that our method significantly outperforms the finetuning scheme, and obtains comparable performance to the state-of-the-art STR methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/append.tex <==
{\color{blue}
\begin{appendix}
\section{The Sampling Strategy}
Algorithm \ref{alg:generate} shows the sampling strategy in our method.
\begin{algorithm}[h]
	\centering
	%\algsetup{linenosize=\tiny}
	\scriptsize
	\setstretch{1.1} %设置具有指定弹力的橡皮长度（原行宽的1.35倍）
	\caption{The sampling strategy.}
	\label{alg:generate}
	\begin{algorithmic}[1]
		\REQUIRE ~~\\
		A source image $\mathcal{I}^s$ and its labels $\hat{\mathcal{Y}}^s=(\hat{y}_1^s, \dots, \hat{y}_L^s)$, \\
		A target image $\mathcal{I}^t$ and its labels $\hat{\mathcal{Y}}^t=(\hat{y}_1^t, \dots, \hat{y}_{L^\prime}^t)$.
		
		\ENSURE ~~\\
		$\mathcal{G}_i, i\in \{1,2,3,4\}$; \\
		%\STATE Randomly sample pairs $I^s$, $I^t$ from $\mathcal{I}^s \times \mathcal{I}^t$,\\
		%\label{ code:fram:extract }
		\STATE Encoding $\mathcal{I}^s$ and $\mathcal{I}^t$ as
		$CR^s=(CR_1^s, \dots, CR_L^s)$ and
		$CR^t=(CR_1^t, \dots, CR_L^t)$, respectively.\\
		%\label{code:fram:trainbase}
		
		\STATE Sampling all pairs of represented characters $CR^s \times CR^t$ to obtain $\mathcal{S}_2$ or $\mathcal{S}_4$:
		\begin{equation}
		\mathcal{S}_k = \left\lbrace CR_i^s, CR_j^t \right\rbrace,\nonumber
		\end{equation}
		where $k$=2 if $\hat{y}_i^s$ = $\hat{y}_j^t$, otherwise $k$=4.
		
		\STATE Sampling all pairs from $CR^s \times CR^s$ to obtain $\mathcal{S}_1$ or $\mathcal{S}_3$:
		\begin{equation}
		\mathcal{S}_k = \left\lbrace CR_i^s, CR_j^s \right\rbrace,\nonumber
		\end{equation}
		\label{code:fram:add}
		where $k$=1 if $\hat{y}_i^s$ = $\hat{y}_j^s$, otherwise $k$=3.
		
		%\STATE Generate pairs of group 1 and 3 as step (\ref{code:fram:add}).
		%\label{code:fram:select}
		\STATE Collecting all pairs $\mathcal{S}_i$ into $\mathcal{G}_i,i\in \{1,2,3,4\}$.
	\end{algorithmic}
\end{algorithm}

\section{The Effect of IA}
In this work, we treat features generated by the attention model as the corresponding character features, but this assumption may be invalid with the existence of the \emph{attention drift} problem. Here, we expect the IA process can alleviate this problem. We define Character Accuracy(ChaAcc) as follow:
\begin{equation}
ChaAcc = \frac{P(y,gt)}{|gt|}
\label{eq:cha_acc}
\end{equation}
where $y$ is the predicted text and $gt$ is the ground truth, and the function $P()$ returns the number of characters at the same position between $y$ and $gt$. We think it will get higher performance at ChaAcc when the features correspond to the characters. Then we execute experiments on the settings as in Table \ref{tab:special_dataset}. The ChaAcc results are presented in Table \ref{tab:character_dataset}. 
In the results of IC03 and IC13, it shows the IA process outperforms the others. And in the results on SVT and IC15, the results of FASDA show the worse performance than FT, because both SVT and IC15 are irregular in order which the attention model is hard to locate the character position. But the IA process can still achieve better performance according to the last two rows of Tab.~\ref{tab:character_dataset}.

\begin{table}[h]
	\centering	
	\begin{tabular}{lcccc}
		\toprule
		Method  & SVT & IC03 & IC13 & IC15 \\
		\midrule
		Source Only     & 51.9 & 68.8 & 66.4 & 36.8  \\
		FT \emph{w/} T  & 56.6 & 72.4 & 68.5  & 42.8 \\
		FT \emph{w/} S+T  & 58.0 & 74.7 & 70.4 & \textbf{43.1}   \\
		\hline
		FASDA-$CR$  & 58.1 & 75.5 & 73.0 & 39.6 \\
		FASDA-$CR^+$   & 58.9 & 76.3 & 73.6 & 40.1   \\
		FASDA-IA-$CR^+$  & \textbf{59.9 }& \textbf{76.9} & \textbf{74.3} & 41.3   \\
		\bottomrule
	\end{tabular}
	\caption{
		%{\color{red}
		{\color{blue} Character Accuracy} results on four benchmarks. 
		%}
	}
	\label{tab:character_dataset}
\end{table}

\section{The Effect of Target Training Set Size}
 We also evaluate the effect of different target training set sizes. Because of the limited training data on public benchmarks, we execute experiments on four collected specific datasets. Here we evaluate Accuracy Increment between the accuracy on FASDA and the accuracy on FT \emph{w/} S+T with the setting similar to Tab. \ref{tab:results-synth} , as shown in Fig.\ref{fig:targetsize}. When the target training samples are insufficient, our method would get more promising performance with the training set size; and when samples are sufficient, the gap would gradually decrease. However, FASDA always outperforms FT w/ S+T.

\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=0.7\textwidth]{images/targetsize_v0.png}
		%\includegraphics[width=0.45\textwidth]{images/arch_v3.png}
	\end{center}
	\caption{TODO}
	\label{fig:targetsize}
\end{figure*}
\end{appendix}
}

==> sections/review.tex <==


\section{Review}
{\color{red}
Paper ID: 3818
Title:    Challenging Text Recognition in Real Scenarios with Few Labeled Samples: A Few-Shot Adversarial Sequence Domain Adaptation Approach 



*** Metareview *** 
*** Review ***
•	Relevance: 7
•	Significance: 7
•	Originality: 6
•	Technical quality: 6
•	Clarity and quality of writing: 6
•	Scholarship: 6
•	Overall score: 6
•	Confidence: 7
- Comments to Authors :

In this article, the authors developed a few-shot adversarial sequence domain adaptation (FASDA) technique to solve the sequence level domain adaptation problem in scene text recognition task. Instead of representing each sequence, each character of the sequence is represented in high level feature by proposing a well designed attention mechanism without explicitly splitting sequences to characters. Finally, the authors designed adversarial learning approach which can maximize the character level confusion between the source domain and the target domain and boost the performance of scene text recognition in real scenarios. The authors experimentally showed that their approach is comparable to the  state-of-the-art techniques.


1. The proposed approach introduced a new solution i.e. few-shot adversarial sequence domain adaptation (FASDA) to solve sequence level domain adaptation problems in scene text recognition.


2. Instead of character annotation, the authors designed an attention mechanism to represent each character in the sequence in high level feature with considering sequence level annotation. This concept reduces the human efforts for charateracter level annotation.


3. Design of adversarial learning approach with few labeled target samples which can maximize the character level confusion between the source domain and the target domain to reduce the domain bias and boost the performance of scene text recognition in real scenarios.
4. The article gives detailed explanations about the proposed idea and discussions about each component of the proposed approach.


5. The authors have done extensive experiments on various benchmark data sets and compare performance of their approach with state-of-the-arts to establish effectiveness of their approach in scene text recognition task.


Concerns:


1. Last paragraph of Section “ 3.1 Weakly-supervised Character Feature Representation”, the authors wrote “Then, we capture …...with only sequence-level annotations”. However, in Eq (5), “ytis the ground truth of t-th character …….”. The authors claimed that they considered only sequence-level annotation to represent each character of the sequence in high level feature then ytcan not be the ground truth of t-th character. Please clarify it.    


2. Why the authors select only three specific datasets from available four specific datasets for “Domain adaptation by specific ----> specific” experiment? The authors should explain it.


3. The authors didn’t mention how many target labeled samples are used for “Comparison with the state-of-the-art” experiment. It is required for establish the authors claim.       





*** Review ***
•	Relevance: 9
•	Significance: 7
•	Originality: 8
•	Technical quality: 7
•	Clarity and quality of writing: 6
•	Scholarship: 6
•	Overall score: 7
•	Confidence: 5 
- Comments to Authors :

This paper presents a few-shot adversarial sequence domain adaptation approach for scene text recognition. The core idea of the paper is to combine attention, which provides character-level detection, and an multi-class discriminator that is confused with adversarial learning, thus reducing domain bias. The results on popular benchmarks demonstrate the goodness of the approach.
In my opinion, this is a good piece of research, although writing can (and should) be improved for a better clarity. I found it especially confusing Section 3.1-Inclusive attending process.
I might have missed something but it is not clear how the approach actually learns the character labels. As far as I understand, Section 3.2 only explains how to reduce domain bias.
Few details are given as regards how and why authors selected the network hyper-parameters. They are just mentioned (but not justified or explained) in Section 4.2.
I miss some comparison with unsupervised domain adaptation. For instance, the work "Ganin, Yaroslav, and Victor Lempitsky. "Unsupervised Domain Adaptation by Backpropagation." International Conference on Machine Learning. 2015." can be easily applied to scene text recognition.
Please add labels to the axes of figure 2.
Please, follow rules for writing mathematical notation (e.g., CR is read as 'C times R')
I found some typos:
•	"labeled samples is deadly lacked"
•	"eaxmple", "encods"
•	"no any"





*** Review ***
•	Relevance: 10
•	Significance: 9
•	Originality: 6
•	Technical quality: 8
•	Clarity and quality of writing: 7
•	Scholarship: 9
•	Overall score: 5
•	Confidence: 6 
- Comments to Authors :

A few-shot adversarial sequence domain adaptation (FASDA) approach has been proposed in this manuscript to solve the sequence-level domain adaptation problem in STR, which is to some extent interesting. Meanwhile, some competitive experiment results has been obtained on the public datasets (e.g., SVT, IC03, et al). However, it still has some problems:
(1) In my understanding, the idea of this paper is unsupervised characters localization + FADA. Unsupervised characters localization is performed by an attention mechanism. Therefore, it is a character-level domain adaptation. I think there is a big gap between the character-level and the sequence-level domain adaption in STR.
(2) The motivation and organization of this paper are not quite clear. For example, the two problems the author mentioned is general for all the STR methods. The authors list three groups of methods with their limitations in the introduction section, but I think most of them should be in the related work section. 
(3) In section 4.4, the competitive experiments has been designed to verify the effectiveness of domain adaptation, some detail information should be provided (e.g., specific to specific).
(4) The pretrained source model only obtain 0% accuracy, the results need some thought, why? the authors need to perform extensive experiments to prove.
(5) In section 3.2, four categories of character pairs have been selected, some reasons should been given in the manuscript.






*** Review ***
•	Relevance: 7
•	Significance: 4
•	Originality: 4
•	Technical quality: 3
•	Clarity and quality of writing: 4
•	Scholarship: 3
•	Overall score: 4
•	Confidence: 7 
- Comments to Authors :

In this paper, the authors develop a few-shot adversarial domain adaptation (FASDA) approach, which combines weakly-supervised character feature representation and few-shot adversarial learning. The weakly-supervised character feature representation is learnt by CNN-LSTM network with the attention model [1,2]. The few-shot Adversarial adaptation approach [3] is exploited to tackle the training data shortages in scene text recognition. However, I think the effectiveness of FASDA is limited.

(1) The results of FASDA in Table 5 are lower than other methods including the baseline model [1] of FASDA, which cannot prove the effectiveness of FASDA.

(2) This method generates a sequence of character-level samples in order to exploit the few-shot adversarial learning strategy [1]. However, it seems that the character-level samples generated by weakly supervised method are unreliable. The authors should give more experiments to verify the reliability of the samples.

(3) It is not clear that how the inclusive attending process works and how to generate character-level samples. I suggest adding more illustrations and figures to clarify the generation of character-level samples. Please show the comparisons between inclusive attending process and other methods which aim to tackle attention drift issue (eg. [1]).

(4) Why randomly choose 150 images form each public benchmark as the target domain in the experiments in Table 2. Please clarify the effect of the size of target domain dataset under finetuning and supervised domain adaptation in Table 3.

(5) Writing in the paper is not very good. The presentation of the paper needs to be improved, especially for grammar and typos. Eg. 1). each public benchmarks(benchmark); 2) It does image-level adaptation.3)FASDA can always more significantly boost.

[1] Cheng Z, Fan B, Xu Y, et al. Focusing Attention: Towards Accurate Text Recognition in Natural Images[J]. 2017.

[2] Shi B, Wang X, Lyu P, et al. Robust Scene Text Recognition with Automatic Rectification[J]. 2016.

[3] Motiian S , Jones Q , Iranmanesh S M , et al. Few-Shot Adversarial Domain Adaptation[J]. 2017.
}

